Domain Adaptation for Satellite-Borne Hyperspectral Cloud Detection

The advent of satellite-borne machine learning hardware accelerators has enabled the on-board processing of payload data using machine learning techniques such as convolutional neural networks (CNN). A notable example is using a CNN to detect the presence of clouds in hyperspectral data captured on Earth observation (EO) missions, whereby only clear sky data is downlinked to conserve bandwidth. However, prior to deployment, new missions that employ new sensors will not have enough representative datasets to train a CNN model, while a model trained solely on data from previous missions will underperform when deployed to process the data on the new missions. This underperformance stems from the domain gap, i.e., differences in the underlying distributions of the data generated by the different sensors in previous and future missions. In this paper, we address the domain gap problem in the context of on-board hyperspectral cloud detection. Our main contributions lie in formulating new domain adaptation tasks that are motivated by a concrete EO mission, developing a novel algorithm for bandwidth-efficient supervised domain adaptation, and demonstrating test-time adaptation algorithms on space deployable neural network accelerators. Our contributions enable minimal data transmission to be invoked (e.g., only 1% of the weights in ResNet50) to achieve domain adaptation, thereby allowing more sophisticated CNN models to be deployed and updated on satellites without being hampered by domain gap and bandwidth limitations.

==> notes/notes_law.tex <==
%- - - - - - - - - - - - - - - -
\cite{ganin2016domain}

Defines unsupervised domain adaptation in Sec. 3.

Embeds domain adaptation into the process of learning representation.

Based on the theory that a good representation for cross-domain transfer is one for which an algorithm cannot learn to identify the domain of origin of the input observation.

Learning features that combine (i) discriminativeness and (ii) domain-invariance, by jointly optimizing the underlying features as well as two
discriminative classifiers operating on these features: (i) the \emph{label predictor} that predicts class labels and is used both during training and at test time and (ii) the \emph{domain classifier} that discriminates between the source and the target domains during training.

Optimisation: minimises the loss of the label classifier and maximises the loss of the domain classifier.

Not reviewed in \cite{fang2023source}.

Although not source-free, classified as intra-domain adversarial alignment in \cite{yu2023comprehensive}.

Although not source-free, classified as virtual domain alignment in \cite[p. 10]{liang2023comprehensive}: Once the source distribution is estimated, it is essential to seek virtual domain alignment between the proxy source domain and the target domain for knowledge transfer.

%- - - - - - - - - - - - - - - -
\cite{li2017revisiting}

Proposed adaptive batch normalisation (AdaBN).

DNNs excel at capture dataset bias, often leading to overfitting.

%- - - - - - - - - - - - - - - -
\cite{mateogarcia2020transferring}

Domain adaptation transformation of Lansdsat-8 data to resemble Proba-V images in terms of both spectral and spatial characteristics.

Taking advantage of existing publicly available cloud masking labeled datasets, creates cloud detection models for new satellites, without the burden of collecting and labeling a large dataset of images.

Three classes of experiments:
\begin{itemize}
    \item transductive transfer learning from Landsat-8 to Proba-V, where only Landsat-8 annotated data is used to develop a model that works in the Proba-V domain;
    \item transductive transfer learning from Proba-V to Landsat-8, where labeled Proba-V data is used to train a cloud detection model for Landsat-8; and
    \item inductive transfer learning from Landsat-8 to Proba-V, where few Proba-V labeled images together with the annotated Landsat-8 dataset are used to generate a cloud detection model for Proba-V.
\end{itemize}

%- - - - - - - - - - - - - - - -
\cite{mateogarcia2021cross}

Trains model on one sensor and uses the model on another sensor; specifically, cloud detection models trained in Landsat-8 data increase cloud detection accuracy in Proba-V.

Uses cycle-consistent generative adversarial (cycleGAN) domain adaptation framework to find a \emph{domain adaptation transformation} from the Proba-V domain to the Landsat-8 upscaled domain that removes noise and saturation of Proba-V images while preventing artifacts on the resulting images.

%- - - - - - - - - - - - - - - -
\cite{segalrozenhaimer2020cloud}

Use a combination of CNN and domain-adversarial training~\cite{ganin2016domain} methods to allow for better transferability of our cloud detector mask from WV-2 to Sentinel-2.

%- - - - - - - - - - - - - - - -
\cite{wang2021tent}

Minimises Shannon entropy of model predictions by modulating features.

Repurposes the BN layer of the source model.

%- - - - - - - - - - - - - - - -
\cite{chen2022update}

%- - - - - - - - - - - - - - - -
\cite{zou2022learning}

Contributes an unsupervised domain adaptation (UDA), based on BatchNorm calibration methods, to address domain shift in out-of-distribution environments.

Two core components:
- Instead of a manually designed BatchNorm calibration rule, a learnable module.
- Leverages strong data augmentation to simulate random domain shifts for learning the calibration rule.

Code provided at \url{https://yuliang.vision/InstCal/}.

\emph{Domain generalisation} learns invariant representations using multiple source domains, but result far from optimal for an unseen target domain.

\emph{Test-time adaptation}: (1) optimise model parameters at test time with a proxy task; (2) optimisation-free BatchNorm calibration. These require backprop.

Contributed method is BatchNorm calibration (an instance of test-time adaptation), where the calibration rule is learned from source-domain data.

Is test-time optimisation used or not?

%- - - - - - - - - - - - - - - -
\cite{hong2023mecta}

Proposed memory-economical continual adaptation (MECTA) that conserve intermediate caches in terms of batch size, channel size, and layer size.

Tricks:
- Shift-aware forget gate?
- Test-time pruning that stochastically removes channels of intermediate results? The simple norm layer structure is ready to be plugged into various networks to replace batch-normalization.

Continual test-time adaptation (CTA) algos like Tent and EATA are memory-consuming, not suitable for small devices.

During forwarding, the MECTA Norm (1) stabilizes the normalisation-statistic estimation via shift-aware moving-average from small batches, (2) randomly drops caches by channel admitting sparse gradient descent without knowing gradient in advance, and (3) maintains caches only for layers on demand of training.

%- - - - - - - - - - - - - - - -
\cite{liang2023comprehensive}

Terminology misuse is rife in the literature.

Domain adaptation (DA) is not domain generalisation, which tries to learn a model using data from one or multiple source domains that can generalise well to any out-of-distribution target domain.

Traditionally, domain adaptation leverages labeled data from a source domain to learn a classifier for an unlabeled target domain with a different distribution, in a/the transductive learning manner (Sec. 2.1).

Defines test-time adaptation (TTA) as adapting a pre-trained model from the source domain to unlabeled data in the target domain before making predictions.

Classifies TTA into 4 categories: 
\begin{itemize}
    \item Test-time (source-free) domain adaptation (TTDA): Uses $m$ test minibatches for multi-epoch adaptation before generating final predictions.
    \item Test-time batch adaptation (TTBA): Individually adapts a pre-trained model to one or few instances. Predictions for each minibatch are independent of the other minibatches.
    \item Online test-time adaptation (OTTA): Adapts the pre-trained model to the target data in an online manner, which each minibatch can only be observed once.
    \item Test-time prior adaptation (TTPA): Addresses label shift rather than data shift.
\end{itemize}

Note in the classification above, test-time adaptation $\neq$ test-time \emph{domain} adaptation (TTDA).

Related to continual learning (or continuous learning, or lifelong leaning) and meta learning.

Data distribution shift and the covariate shift assumption specified on p. 3.

SFDA formally defined through Definition 2. All test data (target data) are required to be seen during adaptation.

Pseudo-labeling (Sec. 3.2.1): The pseudo labels of target data are inaccurate under domain shift, but improvements can be made: (1) by denoising; (2) by filtering out inaccurate pseudo labels with weighting; (3) by developing a robust divergence measure.

%- - - - - - - - - - - - - - - -
\cite{yu2023comprehensive}

Benchmark datasets? (i) Office-31, (ii) Office-home, (iii) VisDA.

Domain shift: conditional shift, covariate shift, label shift, concept shift.

Unsupervised domain adaptation (UDA) uses in general both source-domain and target-domain data: (1) those that ``align'' source-domain and target-domain distributions, (2) those that learn domain-invariant feature representations through adversarial learning. Examples: \cite{ganin2015unsupervised} and \cite{ganin2016domain}.

If Yu et al.'s defintion of UDA is true, then the term ``source-free UDA''~\cite{fang2023source} is inconsistent.

SFDA: (1) data-based, (2) model-based. Note family tree in Fig. 2.

Domain reconstruction methods (see Fig. 4): (i) virtual domain generation, (ii) intra-domain adversarial alignment, (iii) perturbed domain supervision.

The classification tasks dominate the research of SFDA. Most common SFDA algorithms are of the pseudo-labelling type.

Domain divergence is hard to measure in the source-free setting.

Driven mostly by intuition and empirical success.

DA categorised based on relation between source and target domains: (i) partial DA, (ii) open-set DA, (iii) multi-source DA, and (iv) multi-task DA.

Table 1 differentiates between test-time DA and source-free DA.

%- - - - - - - - - - - - - - - -
\cite{fang2023source}

%- - - - - - - - - - - - - - - -
\cite{zhou2023domain}

Domain generalization (DG) aims to achieve OOD generalization using only source data for model learning.

Domain shift is the distribution shift between a set of training (source) data and a set of test (target) data.

See Table 2 for the differences between domain generalisation and domain adaptation etc.

%- - - - - - - - - - - - - - - -
\cite{ruzicka2023fast}

Variational autoencoder model called RaVAEn trained on Sentinel-2 L1C data from the WorldFloods dataset.

Pre-trained encoder used for few-shot learning.

Cloud detection by per-tile classification.
